VideoCrafter2: Overcoming Data Limitations for High-Quality Video Diffusion Models

Text-to-video generation aims to produce a video based on a given prompt. Recently, several commercial video models have been able to generate plausible videos with minimal noise, excellent details, and high aesthetic scores. However, these models rely on large-scale, well-filtered, high-quality videos that are not accessible to the community. Many existing research works, which train models using the low-quality WebVid-10M dataset, struggle to generate high-quality videos because the models are optimized to fit WebVid-10M. In this work, we explore the training scheme of video models extended from Stable Diffusion and investigate the feasibility of leveraging low-quality videos and synthesized high-quality images to obtain a high-quality video model. We first analyze the connection between the spatial and temporal modules of video models and the distribution shift to low-quality videos. We observe that full training of all modules results in a stronger coupling between spatial and temporal modules than only training temporal modules. Based on this stronger coupling, we shift the distribution to higher quality without motion degradation by finetuning spatial modules with high-quality images, resulting in a generic high-quality video model. Evaluations are conducted to demonstrate the superiority of the proposed method, particularly in picture quality, motion, and concept composition.

==> fig_tex/fig_comp_sota.tex <==
\if \animation 1
\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-001.png}
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/526/526-}{0}{15} 
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/525/525-}{0}{15}
  \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-002.png}
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/528/528-}{0}{15} 
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/531/531-}{0}{15} \\
  \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-003.png}
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/532/532-}{0}{15} 
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/533/533-}{0}{15}
  \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-004.png}
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/545/545-}{0}{15} 
  \animategraphics[width=0.15\linewidth]{8}{gif/ADvsAZ/549/549-}{0}{15}

  \caption{AnimateDiff v.s. AnimateZero }
  \vspace{-0.1cm}
\label{fig:ADvsAZ} 
\end{figure*}

\else
\begin{figure*}[ht]
  \centering
  \begin{tabular}{c@{\hspace{0.3em}}c@{\hspace{0.3em}}c@{\hspace{1.2em}}c@{\hspace{0.3em}}c@{\hspace{0.3em}}c}
  Generated Images & AnimateDiff~\cite{guo2023animatediff} & AnimateZero (ours) & Generated Images & AnimateDiff~\cite{guo2023animatediff} & AnimateZero (ours)\\
    \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-001.png}&
    \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/526/526-0.png}&
     \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/525/525-0.png}&
     \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-002.png}&
      \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/528/528-0.png}&
       \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/531/531-0.png}
       \\
       \multicolumn{3}{c}{\textit{``1girl, jewelry, upper body, earrings, ...''}} & \multicolumn{3}{c}{\textit{``1girl, jewelry, upper body, earrings, ...''}}\\
       \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-003.png}&
       \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/532/532-0.png}&
     \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/533/533-0.png}&
     \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/mix-004.png}&
      \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/545/545-0.png}&
       \includegraphics[width=0.15\linewidth]{gif/ADvsAZ/549/549-0.png}\\
       \multicolumn{3}{c}{\textit{``1girl, jewelry, upper body, earrings, ...''}} & \multicolumn{3}{c}{\textit{``1girl, jewelry, upper body, earrings, ...''}}
    \end{tabular}

  \caption{Qualitative comparison results between AnimateDiff~\cite{guo2023animatediff} and our proposed AnimateZero.}
  \vspace{-0.1cm}
\label{fig:ADvsAZ} 
\end{figure*}

\fi

==> fig_tex/fig_disentangle_module.tex <==
\if \animation 0

\begin{figure}[t]
  \centering
  \setlength{\tabcolsep}{0.1pt} % Remove cell spacing
  \begin{tabular}{>{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{3.8cm} >{\centering\arraybackslash}m{3.8cm} }
     & \textit{a dog running in forest } & a woman dancing in a hall \\
    \rotatebox{90}{ \small P-Spa\&Temp-LORA } &
    % \animategraphics[width=\linewidth]{8}{fig/comp_sota/0/0-}{1}{16}&
    \animategraphics[width=\linewidth]{8}{fig/comp_sota/0/0-}{1}{16}&
    \animategraphics[width=\linewidth]{8}{fig/comp_sota/0/0-}{1}{16} \\
    \rotatebox{90}{ \small F-Temp-DIR } &
    \includegraphics[width=\linewidth]{example-image-a} &
    \includegraphics[width=\linewidth]{example-image-b}  \\
    \rotatebox{90}{ \small F-Spa-DIR } &
    \includegraphics[width=\linewidth]{example-image-a} &
    \includegraphics[width=\linewidth]{example-image-b}  \\
    \rotatebox{90}{ \small F-Spa\&Temp-DIR } &
    \includegraphics[width=\linewidth]{example-image-a} &
    \includegraphics[width=\linewidth]{example-image-b}  \\
  \end{tabular}
  \caption{Finetuning different modules based on the fully trained T2V base model.  \textit{Best viewed with Acrobat Reader. Click the images to play the video clips.}}
  \label{fig:disentangle-module}
\end{figure}

\else

\begin{figure}[t]
  \centering
  \setlength{\tabcolsep}{0.1pt} % Remove cell spacing
  \begin{tabular}{>{\centering\arraybackslash}m{0.5cm} >{\centering\arraybackslash}m{3.8cm} >{\centering\arraybackslash}m{3.8cm} }
     & \textit{a dog running in forest } & a woman dancing in a hall \\
    \rotatebox{90}{\small P-Spa\&Temp-LORA } &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/fix-1k/0012_00.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/fix-10k/0012_00.jpg}  \\
    \rotatebox{90}{\small F-Temp-DIR } &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/full-1k/0012_00.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/full-10k/0012_00.jpg}  \\
    \rotatebox{90}{\small F-Spa-DIR } &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/fix-1k/0012_00.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/fix-10k/0012_00.jpg}  \\
    \rotatebox{90}{\small F-Spa\&Temp-DIR } &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/full-1k/0012_00.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_lora_spatial/full-10k/0012_00.jpg}  \\
  \end{tabular}
  \caption{Finetuning different modules based on the fully trained T2V base model.  \textit{Best viewed with Acrobat Reader. Click the images to play the video clips.}}
  \label{fig:disentangle-module}
\end{figure}

\fi

==> fig_tex/fig_teaser.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{fig/comp_sota/0/0-1.png}
    \caption{To overcome data limitations for training high-quality video models, we propose to disentangle motion from appearance at the data level, \textit{i.e.,} low-quality videos for motion learning and high-quality images for appearance promotion. (a) Conventional solution with high-quality videos. (b) Our disentanglement solution. }
    \label{fig:teaser}
\end{figure}

==> fig_tex/fig_teaser_sample.tex <==
\if \animation 1

\begin{figure*}[ht]
  \centering
  \setlength{\tabcolsep}{0.3pt} % Remove cell spacing
  \begin{tabular}{>{\centering\arraybackslash}m{5.8cm} >{\centering\arraybackslash}m{5.8cm} >{\centering\arraybackslash}m{5.8cm} }
     {\small \textit{prompt1} & {\small  \textit{prompt1} } & {\small \textit{prompt1} } \\
    % \animategraphics[width=\linewidth]{8}{fig/comp_sota/0/0-}{1}{16}&
    \includegraphics[width=\linewidth]{fig/comp_dir_part/spatial_temp_lora/0036_0.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_dir_part/temp/0036_0.jpg} &
    \includegraphics[width=\linewidth]{fig/comp_dir_part/spatial/0036_0.jpg}  \\
  \end{tabular}
  \caption{Give a text prompt, our method can generate a video with high visual quality and accurate text-video alignment.  Note that it is trained with only low-quality videos and high-quality images. \textit{Best viewed with Acrobat Reader. Click the images to play the video clips.}}
  \label{fig:teaser}
\end{figure*}


\else

\begin{figure*}[ht]
  \centering
  \setlength{\tabcolsep}{0.3pt} % Remove cell spacing
  \begin{tabular}{>{\centering\arraybackslash}m{5.8cm} >{\centering\arraybackslash}m{5.8cm} >{\centering\arraybackslash}m{5.8cm} }
     {\small \textit{prompt1}} & {\small  \textit{prompt2} } & {\small \textit{prompt3} } \\
    % \animategraphics[width=\linewidth]{8}{fig/comp_sota/0/0-}{1}{16}&
    \animategraphics[width=\linewidth]{8}{fig/comp_dir_part/spatial_temp_lora/0036_}{0}{15}&
    \animategraphics[width=\linewidth]{8}{fig/comp_dir_part/temp/0036_}{0}{15}&
    \animategraphics[width=\linewidth]{8}{fig/comp_dir_part/spatial/0036_}{0}{15} \\
  \end{tabular}
  \caption{Give a text prompt, our method can generate a video with high visual quality and accurate text-video alignment.  Note that it is trained with only low-quality videos and high-quality images. \textit{Best viewed with Acrobat Reader. Click the images to play the video clips.}}
  \label{fig:teaser}
\end{figure*}


\fi

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/exp_table.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{lcc}
\toprule
Method & Aesthetic Score & Technical Score \\
\midrule
Base-T2V & 46.55 & 51.76 \\
ALL-spatial & 82.57 & 70.35 \\
\bottomrule
\end{tabular}

}
\caption{
Caption goes here
}
\vspace{-0.05in}
\label{tab:template}
\end{table}

